K-theory of Gieseker variety and type A cyclotomic Hecke algebra

We give an algebraic description of the equivariant K-theory of Gieseker varieties. Our main result identifies the equivariant K-theory of the Gieseker space with the Jucys--Murphy center of the cyclotomic Hecke algebra, over the equivariant K-theory of a point. The construction is inspired by the proof of the Hikita--Nakajima conjecture for Gieseker spaces given by the first and third authors. We discuss consequences for the center of cyclotomic Hecke algebras and for specializations to q=1 and to roots of unity. In particular, we relate K-theory of affine type A quiver varieties with the centers of the corresponding blocks of specialized cyclotomic Hecke algebras. This last result strengthens the correspondences obtained by the second author in earlier work.

==> section/Notation.tex <==
The following is a list of all the notation that we use:
\begin{itemize}
    \item $\cotrepspace$ : Representation space \verb|\cotrepspace|
    \item $\Gie(n,r)$ : Gieseker space \verb|\Gie(n,r), \Gis|
    \item $\mathcal{T}$ : maximal diagonal torus of $\SL_2$ $\times$ maximal diagonal torus of $\GL_r$ \verb|\mathcal{T}, \torus|
    \item $\mathcal{R}:=\C[q^{\pm 1}, Q_1^{\pm 1},\dots,Q_r^{\pm 1}]$ : $\mathcal{T}$-equivariant $K$-theory of a point \verb|\mathcal{R}, \CR|
    \item $\Heck_{n,r}$ : Cyclotomic Hecke algebra\verb|\Heck_{n,r}|
    \item $L_1,\dots, L_n$ : Jucys-Murphy elements of $\Heck_{n,r}$ \verb||
    \item $\ZJM$ : Jucys-Murphy center of $\Heck_{n,r}$ \verb|\ZJM|
    \item $\mathcal{P}_n^r$ : set of all $r$-multipartitions of $n$ \verb|\mathcal{P}_n^r, \mpart|
    \item $\lbb$ : a multipartition \verb|\lbb|
    \item $\CV$: tautological vector bundle \verb|\CV|
    \item $\KTmpart$: our mpart algebra \verb|K_{\mathcal{T}}(\mathcal{P}^r_n), \KTmpart|
    \item $\KTGis$: our algebra \verb| K_{\mathcal{T}}(\mathcal{G}(n,r)), \KTGis |
\end{itemize}
